1-2-3-Go! Policy Synthesis for Parameterized Markov Decision Processes via Decision-Tree Learning and Generalization

Despite the advances in probabilistic model checking, the scalability of the verification methods remains limited. In particular, the state space often becomes extremely large when instantiating parameterized Markov decision processes (MDPs) even with moderate values. Synthesizing policies for such \emph{huge} MDPs is beyond the reach of available tools. We propose a learning-based approach to obtain a reasonable policy for such huge MDPs. The idea is to generalize optimal policies obtained by model-checking small instances to larger ones using decision-tree learning. Consequently, our method bypasses the need for explicit state-space exploration of large models, providing a practical solution to the state-space explosion problem. We demonstrate the efficacy of our approach by performing extensive experimentation on the relevant models from the quantitative verification benchmark set. The experimental results indicate that our policies perform well, even when the size of the model is orders of magnitude beyond the reach of state-of-the-art analysis tools.

==> 6_discussion.tex <==
\section{Discussion}

%WE ARE BETTER ALSO FOR OTHER REASONS!

While the main focus of our approach is to generate strategies and lower bounds for MDP where other techniques fail, we additionally generate strategies that are much more explainable than standard look-up tables. We show the results in Section \ref{sec:dt-sizes}.

Whereas our approach is straightforward, there are some fine adjustments that had to be made. We explain the parameters and choices that we did in Section \ref{sec:dt-learning-details}.


\subsection{DT sizes and explainability} \label{sec:dt-sizes}

It is known that decision trees can represent strategies in less space than a look-up table needs \cite{AshokJJKWZ20a}.
But apart from the reduction of memory consumption, these strategies are more explainable \cite{BrazdilCCFK15, AshokKLCTW19, KiesbyeGAK22}. 
In contrast to having millions of lines in a state-action lookup table, decision trees capture the inherent structure and generalize, while still representing the same strategy.
We see in our results that this principle is still true for the models in our experiments.
In Table \ref{tab:states-dt-sizes}, we show the number of states, i.e. the size of a standard lookup-table, in comparison to the size of our best decision trees. We refer to size here as the total number of nodes in the tree, including decision- and leaf-nodes.
In Table \ref{tab:states-dt-sizes-full}, we show the sizes of the decision-trees for each property.

For all models, the decision tree is several magnitudes smaller than the number of states. In most cases the decision tree has less than 100 nodes, which is a size that a human can easily parse and interpret. 
Note that for many models, the optimal decision tree has even size 1, which means there is a very simple strategy that our approach can find.


%For some models, our DT is really small. We understand philosopher, and X, Y and Z are within reach. Almost all are smaller than 1000.
%Note that [Jonis+Kush] managed to analyse DTs with million size and use this to adapt and validate their model. This means it is feasible to analyse our strats, in contrast to the million of line state-action lookup table that the others can give.


\begin{table}[!htp]\centering
	\scriptsize
	\begin{tabular}{ll|rr}\toprule
		Model &Parameter &\#states &\#nodes \\\midrule
		consensus&N=8 &61,018,112 &31-60343 \\
		&N=10 &2,761,248,768 & 31-45\\
		csma &3\_4 &1,460,287 &1 \\
		&3\_6 &84,856,004 &1-35 \\
		&4\_4 &133,301,572 &1-35\\
		&4\_6 &39,051,159,469 &1 \\
		&4\_6 &39,051,159,469 &1 \\
		firewire &deadline=200 &6,931,981 &1-13 \\
		&deadline=600 &87,025,687 &1 \\
		mer &N=3000 &17,722,564.00 &43 \\
		&N=6000 &35,443,564.00 &43 \\
		pacman &MAXSTEPS=60 &38,786,521 &1 \\
		&MAXSTEPS=100 &79,440,921 &321 \\
		philosopher &N=10 &N/A &327 \\
		&N=30 &N/A &327 \\
		&N=80 &N/A &327 \\
		rabin  &N=6 &N/A &87 \\
		&N=10 &358,055,586,147,376 &55 \\
		wlan with COL=0 &MAX\_BACKOFF=6 &5,007,548 &1-79 \\
		&MAX\_BACKOFF=10 &N/A &1-79 \\
		wlan\_dl  &MAX\_BACKOFF=5 &9,633,089 &1 \\
		&MAX\_BACKOFF=6 &10,131,465 &19 \\
		&MAX\_BACKOFF=10 &N/A &19 \\
		\bottomrule
	\end{tabular}
	\caption{State size and Decision-Tree size}
	\label{tab:states-dt-sizes}
\end{table}

\subsection{Analyzing our approach in detail}\label{sec:dt-learning-details}
In the following we differentiate the following dimensions:
\begin{itemize}
	\item the 9 models and the consequently 40 combinations of model, parameter and property% (40 model-scaling-parameter-property combinations)
	\item the decision-tree learning method
%	\item DT learner: dtControl, sklearn or MLpack
	\item the parameter we use for our learning approach
%	\item params: the parameters we inserted for learning in our approach (e.g. philosophers2 or (2 and 4) or (2, 4 and 6) ...)
\end{itemize}

The choice of models and parameters were done based on QComp to evaluate our approach on a reasonable set. The other two parameters, however, were chosen after a thorough investigation.

\subsubsection{Which decision-tree learning method to use}\label{sec:disc-dt-learners}

When learning a decision tree, there are several possibilities that come to mind. The most common approach is to use the Python-library Sklearn \cite{scikit-learn}. Additionally, we used dtControl \cite{AshokJJKWZ20a} because it shows promising results in creating small and correct decision trees for strategies, and MLPack \cite{CurtinELMGZ18} because it is a fast C++-library that works well together with our implementation in Storm. 

We evaluate each approach on all combinations of models, properties and parameter and on a set of learning-parameters and evaluate the difference of the true value to the value that our strategy achieves. 

We found that the approaches almost always achieve the same value. Only on two models, Consensus and Rabin, dtControl could outperform MLPack and Sklearn. 
The complete evaluation can be found in Appendix \ref{app:learner}.
Therefore, we decided to continue our experiments with dtControl.




%Additionally, line plot.
%X-axis: models
%Y-axis: best trueval-predictval (aka error)
%Three lines, one for each learner.
%(this plot can replace the best params box plot. If dtControl line consistently below the others, good argument to use it)

So far, we have only used standard variants of the proposed algorithms. In future work, we want to see if we can improve our results even further by understanding the tools more and making use of their variety of different approaches.

%We decide that one of them is best, and use that in THE-BIG-TABLE and the following.

%Weird that dtControl is best, since it tries not to generalize, but rather overfit the given data. But maybe the generalizing comes from the unknown states, and it is best to learn the strat on the given states exactly.

%FW: Might try other dtControl variants, like MLEntropy.



\subsubsection{Which parameters to use for learning}

From now on, we consider only dtControl as a fixed learning algorithm. 
Since our approach relies on smaller models to learn a strategy from, we need to specify these models.%, or usually the parameters for the model that we want to learn from.
We want to see if the impact of the choice of these models on the results.

\begin{figure}
	\center
	\includegraphics[width=0.6\textwidth]{images/boxplot_dtcontrol_learnparam_selected.jpg}
	\caption{Boxplot for four selected models. This shows the difference (=error) of the value calculated by our strategy and the true value. The values are accumulated over all possible learning-parameters and for dtControl as a learning algorithm.}
	\label{fig:boxplot-param-selected}
\end{figure}

In Figure \ref{fig:boxplot-param-selected}, we can see box-plots for four selected models that represent a representative selection. We show how the value that our strategy achieves can vary when we use different parameters to learn from. 
Each plot shows the variance of the error, i.e. the difference of the true value to the value achieved by our strategy, for different learning-parameters for one model and property. 
A full plot for models can be found in Figure \ref{fig:boxplot-param-all-dtcontrol}, but the four models were chosen because they can represent the behavior of all others.

For some models, e.g. Consensus, the choice of parameter can have a huge impact. On other models, e.g. Philosophers or Firewire, the parameters have a small impact,. Finally, on many models, e.g. Wlan-Deadline, the parameters have no influence at all. 
The latter happens on 14 of the considered 23 models.

We can conclude that, although the parameters have some impact, in most of the cases, the impact is considerably small. Therefore, it suffices to manually choose a set of parameters to evaluate.
In future work, we want to see if there are efficient ways to see which parameters are a good choice, or make use of hyperparameter-tuning methods from the Machine-Learning-community.




%Fix best learner.

%For each model: Boxplot of value for each param.
%(for other learners could be in appendix)
%(probably only select 4 representative models or sth like that; then say "for X out of Y models, the picture looks like this")

%Expected outcome: it has some impact what we pick. (there is spread in the boxplot)
%There are interesting things such as philosopher generalizing to best strat with 4 but not when one adds 3 or 5.
%More interesting things?

%However, overall the impact is quite limited, the spread in the boxplot usually is small. Thus, in the following, we always use best param. (Do we? Would it be ok?)

%In general, one might try grid search, but handpicking or some random selection seems fine. 
%Domain knowledge can be abused (symmetries, philosopher4 thing explanation?)

==> format/macros.tex <==
% == ALGORITHMS
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
%\algrenewcommand{\algorithmiccomment}[1]{\hskip1.5em \textbackslash *  #1 * \textbackslash}
%\renewcommand{\algorithmiccomment}[1]{\bgroup\hfill\tiny//~#1\egroup}

% == GRAPHICS
%\DeclareGraphicsExtensions{.pdf, .png, .jpg}

% == LATEX
%\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}

% == THEOREMS
%\newtheorem{theo}{Theorem}[section]
%\newtheorem{cor}{Corollary}%[lemma]
%\newtheorem{ass}{Assumption}%[lemma]
%\newtheorem{lem}[theo]{Lemma}

%\def\qedtriangle{\hspace{\stretch1}\ensuremath\triangleleft}
%\def\qedsquare{\hspace{\stretch1}\ensuremath\square}

% == SYMBOLS

\RequirePackage{marvosym}

\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
\DeclarePairedDelimiter\abs{\lvert}{\rvert}

% == BASIC SETS

\newcommand{\Naturals}{\mathbb{N}}
\newcommand{\Reals}{\mathbb{R}}
\newcommand{\Distributions}{\mathcal{D}}
\newcommand{\Paths}{\mathsf{Paths}}


% == OPERATORS

\DeclareMathOperator*{\argmax}{arg\, max}
\DeclareMathOperator*{\argmin}{arg\, min}
\newcommand{\post}{\mathsf{post}}
%\DeclareMathOperator{\leaves}{\mathbin{\mathop{exits}}}
\newcommand{\eqdef}{\vcentcolon=}
\newcommand{\defeq}{=\vcentcolon}

\newcommand{\qee}{\hfill$\triangle$} % quod erat exemplandum % TODO del

% == COMPLEXITY
%\newcommand{\NP}{\mathbf{NP}}
%\newcommand{\NEXP}{\mathbf{NEXP}}
%\newcommand{\PSPACE}{\mathbf{PSPACE}}

% == PROBABILITY
\renewcommand{\Pr}{\mathbb{P}}
\newcommand{\Expectation}{\mathbb{E}}
%\newcommand{\CPT}{\mathbb{C}}

% == MC, MPD, Games
\newcommand{\MDP}{\mathcal{M}}
\newcommand{\initstate}{\bar{s}}
\newcommand{\states}{\mathsf{S}}
\newcommand{\actions}{\mathsf{A}}
%\newcommand{\enActions}{E}
\newcommand{\trans}{\delta}
\newcommand{\gStates}{\mathsf{G}}
\newcommand{\Reach}{\mathsf{Reach}}
\newcommand{\domain}{\mathbb{D}}

% == CPT
%\newcommand{\pweight}{\pi^+}
%\newcommand{\mweight}{\pi^-}
%\newcommand{\utility}{\nu}
%\newcommand{\weight}{w}

% = paths and strategies
\newcommand{\apath}{\rho}
\newcommand{\paths}{\mathsf{Paths}}
\newcommand{\policy}{\sigma}
\newcommand{\policies}{\Sigma}
\newcommand{\prob}{\mathbb{P}}
\newcommand{\opt}{\mathsf{opt}}


% == Tikz
%\newcommand{\drawcirc}{\node[draw,circle,minimum size=.7cm, outer sep=1pt]}
%\newcommand{\drawbox}{\node[draw,rectangle,minimum size=.7cm, outer sep=1pt]}
%\newcommand{\drawdummy}{\node[minimum size=0,inner sep=0]}


\newcommand{\val}{\mathsf{V}}

\newcommand{\todos}[1]{\todo[color=green]{\textbf{Steffi:} #1}}
\newcommand{\todoma}[1]{\todo[color=blue]{\textbf{Maxi:} #1}}
\newcommand{\todoj}[1]{\todo[color=red]{\textbf{Jan:} #1}}
\newcommand{\todomu}[1]{\todo[color=orange]{\textbf{Muqsit:} #1}}

\newcommand\precnum[1]{\tablenum[round-mode=off,table-format=4.1]{#1}}
\newcommand\rndnum[1]{\tablenum[round-mode=figures,round-precision=2,table-format=4.2]{#1}}
\newcommand\precnumnodec[1]{\tablenum[round-mode=off,table-format=4.0]{#1}}
\newcommand\rndnumnodec[1]{\tablenum[round-mode=figures,round-precision=2,table-format=4.0]{#1}}

\newcommand\rednote[1]{\textcolor{red}{\bfseries #1}}
\newcommand\bluechange[1]{\textcolor{blue}{#1}}

\newcommand\tool[1]{{{\scshape #1}\xspace}}
%\newcommand\definetool[2]{\newcommand{#1}{\tool{#2}\xspace}}
\newcommand\definetool[2]{\newcommand{#1}{\tool{#2}\xspace}}
\definetool{\benchexec}{BenchExec}
\definetool{\storm}{Storm}
\definetool{\modes}{MODES}
\definetool{\modest}{MODEST}
\definetool{\prism}{PRISM}

\newcommand{\aminute}{$<$ 1 min}
\newcommand{\anhour}{$<$ 60 min}

\newcommand{\oor}{\textsc{OOR}}
\newcommand{\error}{\textsc{ERROR}}
\newcommand{\rle}{\textsc{RLE}}

\newcommand\notemodest{{$^\sharp$}}

\newcommand\expnum[1]{{\num[round-mode=places,round-precision=2]{#1}}}

\newcolumntype{H}{>{\setbox0=\hbox\bgroup}c<{\egroup}@{}}
\usepackage{pgfplots}
\pgfplotsset{compat=1.18}

% new macros
\renewcommand{\circ}{\bigcirc}
\newcommand{\baseinstances}{\mathcal{B}} 


==> format/spacing.tex <==
% SPACE HACKS
%\titlespacing*{\section}{0pt}{12pt plus 4pt minus 4pt}{12pt plus 2pt minus 2pt}
%\titlespacing*{\subsection}{0pt}{10pt plus 3pt minus 3pt}{10pt plus 2pt minus 1pt}
%\titlespacing\subsubsection{0pt}{8pt plus 2pt minus 2pt}{8pt plus 1pt minus 1pt}

%\renewcommand{\baselinestretch}{0.98} % >=0.97
\advance\textwidth3mm % <= 5mm
\advance\hoffset-1.5mm
\advance\textheight1mm
%\advance\voffset-3mm

%\setlength{\marginparwidth}{3.3cm}
%\setlength{\marginparsep}{0.1cm}
%\setlength{\textfloatsep}{0.8\textfloatsep} % Space below/above a float if its [t]
%\setlength{\intextsep}{0.8\intextsep} % Space below/above a float if its [h]



%\makeatletter
%\renewcommand\section{\@startsection {section}{1}{\z@}%
%      {-2ex \@plus -1ex \@minus -.2ex}% <beforeskip>
%      {1ex \@plus .2ex}% <afterskip>
%      {\normalfont\Large\bfseries\SS@sectfont}}
%\renewcommand\subsection{\@startsection{subsection}{2}{\z@}%
%      {-2ex\@plus -1ex \@minus -.2ex}% <beforeskip>
%      {1ex \@plus .2ex}% <afterskip>
%      {\normalfont\large\bfseries\SS@subsectfont}}
%\makeatother

% Gaps between titles

% \titlespacing*{<command>}{<left>}{<before-sep>}{<after-sep>}
%\titlespacing*{\section} {0pt}{3.5ex plus 1ex minus .2ex}{2.3ex plus .2ex}
% \titlespacing*{\subsection} {0pt}{3.25ex plus 1ex minus .2ex}{1.5ex plus .2ex}
% \titlespacing*{\subsubsection}{0pt}{3.25ex plus 1ex minus .2ex}{1.5ex plus .2ex}
% \titlespacing*{\paragraph} {0pt}{3.25ex plus 1ex minus .2ex}{1em}
% \titlespacing*{\subparagraph} {\parindent}{3.25ex plus 1ex minus .2ex}{1em}

% Alter some LaTeX defaults for better treatment of figures:
% See p.105 of "TeX Unbound" for suggested values.
% See pp. 199-200 of Lamport's "LaTeX" book for details.
%   General parameters, for ALL pages:
\renewcommand{\topfraction}{0.95}	% max fraction of floats at top
\renewcommand{\bottomfraction}{0.95}	% max fraction of floats at bottom
%   Parameters for TEXT pages (not float pages):
% \setcounter{topnumber}{2} % number of floats that can be displayed at the top
% \setcounter{bottomnumber}{2} % number of floats that can be displayed at the bottom
% \setcounter{totalnumber}{4}     % 2 may work better
% \setcounter{dbltopnumber}{2}    % for 2-column pages
% \renewcommand{\dbltopfraction}{0.9}	% fit big float above 2-col. text
\renewcommand{\textfraction}{0.07}	% allow minimal text w. figs
%   Parameters for FLOAT pages (not text pages):
\renewcommand{\floatpagefraction}{0.95}	% require fuller float pages
% N.B.: floatpagefraction MUST be less than topfraction !!
% \renewcommand{\dblfloatpagefraction}{0.7}	% require fuller float pages
% remember to use [htp] or [htpb] for placement


% A good document on space hacks
% http://www-h.eng.cam.ac.uk/help/tpl/textprocessing/squeeze.html


% space left between floats (12.0pt plus 2.0pt minus 2.0pt).
\setlength{\floatsep}{10pt}
% space between last top float or first bottom float and the text (20.0pt plus 2.0pt minus 4.0pt).
\setlength{\textfloatsep}{16pt}
% space left on top and bottom of an in-text float (12.0pt plus 2.0pt minus 2.0pt).
\setlength{\intextsep}{10pt}
%\dbltextfloatsep is \textfloatsep for 2 column output (20.0pt plus 2.0pt minus 4.0pt).
%\dblfloatsep is \floatsep for 2 column output (12.0pt plus 2.0pt minus 2.0pt).
% space above caption (10.0pt).
\setlength{\abovecaptionskip}{10pt}
% space below caption (0.0pt).
\setlength{\belowcaptionskip}{0pt}

==> table-base-instance1.tex <==
\begin{table}[h]
	\renewcommand{\arraystretch}{1.2}
	\setlength\fboxsep{1cm}
	\caption{MDPs in the benchmark set, parameters, choice of base instances, and the size of the generated decision trees}
	\label{table:baseinstance:dtsize}
	\begin{adjustbox}{width=\textwidth,center}
		\begin{tabular}{l|@{\hskip 5mm}p{0.45\textwidth} p{0.3\textwidth}|r}
			\toprule
			Model instance
			& Parameters 
			& \parbox{0.2\textwidth}{Parameter value for base instance} 
			& DT size\\
			\midrule
			\multicolumn{4}{c}{Maximizing Probabilities} \\
			consensus+disagree
			& \parbox{0.2\textwidth}{(N, \#modules),\\(K,Var)}
			& \{(N=2,K=8), (N=3,K=8)\} 
			& 347\\
			\hline
			
			csma+all\_before\_max
			& \parbox{0.2\textwidth}{(N, \#modules),\\(K,Var)} 
			& \{(N=2,K=2), (N=3,K=2)\} 
			& 1\\
			\hline
			
			% SK: Commented out because semantic action labels mess it up
			mer+p1
			& \parbox{0.4\textwidth}{(n, Var),\\(x, Var, probability)} 
			& \parbox{0.2\textwidth}{\{(n=1,x=0.01)\}} 
			& 19\\
			\hline 
			
			philosophers+eat
			& (N, \#modules, number of processes)
			& \{(N=4)\}
			& 109\\
			\hline
			
			zeroconf\_dl+deadline\_max
			& \parbox{0.2\textwidth}{(deadline, Var),\\(K,Var)} 
			& \parbox{0.2\textwidth}{\vspace{3pt}\{(reset=false, \\ N=1000,K=2, \\deadline=50)\}\vspace{3pt}}
			& 1413 \\
			\hline
			
			pnueli-zuck+live
			& (N, \#modules, number of processes)
			& \{(N=3)\}
			& 65\\
			\hline
			
			\multicolumn{3}{c}{Minimizing Probabilities} \\
			consensus+c2
			& \parbox{0.2\textwidth}{(N, \#modules),\\(K,Var)}
			& \{(N=2,K=8), (N=3,K=8)\} 
			& 161\\
			\hline
			
			%			\rednote{csma+all\_before\_min}
			%			& \parbox{0.2\textwidth}{(N, \#modules),\\(K,Var)}
			%			& ??? \\
			%			\hline
			
			csma+some\_before
			& \parbox{0.2\textwidth}{(N, \#modules),\\(K,Var)} 
			& \{(N=2,K=2), (N=3,K=2)\} 
			& 1\\
			\hline
			
			zeroconf\_dl+deadline\_min
			& \parbox{0.2\textwidth}{(deadline, Var),\\(K,Var)} 			
			& \parbox{0.2\textwidth}{\vspace{3pt}\{(reset=false, \\ N=1000,K=2, \\deadline=50)\}\vspace{3pt}} 
			& 377\\
			\hline
			
			firewire+deadline
			& \parbox{0.2\textwidth}{(deadline, Var) , \\ (delay, Var)}
			& \parbox{0.2\textwidth}{\vspace{3pt}\{(deadline=200, \\ delay=3)\}\vspace{3pt}}
			& 1\\
			\hline
			
			pacman+crash
			& {(MAX\_STEPS, Var)}
			& \{(MAX\_STEPS=5)\} 
			& 1\\
			\bottomrule
			
		\end{tabular}
	\end{adjustbox}
\end{table}


==> table-instance-size.tex <==
\begin{table}[t!]
	\renewcommand{\arraystretch}{1.2}
	\setlength\fboxsep{1cm}
	\caption{The size of parameters in our comparison}
	\label{table:instancesize}
	\begin{adjustbox}{width=\textwidth,center}
		\begin{tabular}{l|@{\hskip 5mm}p{0.2\textwidth} p{0.2\textwidth} p{0.2\textwidth}}
			\toprule
			Model instance
			& \aminute
			& \anhour 
			& Beyond \\
			\midrule
			\multicolumn{4}{c}{Maximizing Probabilities} \\
%			consensus+disagree $\uparrow$ \\ (fix N=2)
%			& 
%			&  \\
%			\hline
			
%			consensus+disagree $\uparrow$ \\ (fix K=2)
%			& N=5
%			& N=7
%			& N=13 \\
%			\hline
			
%			csma+all\_before\_max $\uparrow$ \\ (fix N=2)
%			& K=8
%			& K=11
%			& K=13\\
%			\hline
%			
%			csma+all\_before\_max $\uparrow$ \\ (fix K=2)
%			& N=3
%			& N=5 
%			& N=6\\
%			\hline
			
			% SK: Commented out because semantic action labels mess it up
			%			mer+p1
			%			& 
			%			& \\
			
%			philosophers+eat $\uparrow$
%			& N=5
%			& N=21
%			& N=34 \\
%			\hline
%			
%			mer+p1 $\uparrow$ \\ (fix x=0.01)
%			& n=1000
%			& n=21000
%			& n=55000 \\
%			\hline
%			
%			mer+p1 $\uparrow$ \\ (fix n=10)
%			& x=0.89
%			& x=0.89
%			& x=0.89 (NA) \\
%			\hline
%			
%			pnueli-zuck+live $\uparrow$
%			& N=5
%			& N=21
%			& N=34 \\
%			\hline
			
%			zeroconf\_dl+deadline\_max $\uparrow$ \\
%			(fix reset=false,N=1000,K=2)
%			& deadline=200
%			& deadline=1600
%			& deadline=3200\\
%			\hline
			
			\multicolumn{4}{c}{Minimizing Probabilities} \\
			consensus+c2 $\downarrow$ \\ (fix K=2)
			& N=6
			& N=7
			& N=13\\
			\hline
			
			\rednote{csma+all\_before\_min $\downarrow$}
			& \parbox{0.2\textwidth}{(N, \#modules),\\(K,Var)}
			& ??? \\
			\hline
			
			csma+some\_before $\downarrow$ \\ (fix N=2)
			& K=10
			& K=12
			& K=13\\
			\hline
			
			csma+some\_before $\downarrow$ \\ (fix K=2)
			& N=3
			& N=8
			& N=13\\
			\hline
						
%			zeroconf\_dl+deadline\_min $\downarrow$ \\
%			(fix reset=false,N=1000,K=2)
%			& deadline=200
%			& deadline=1600
%			& deadline=3200\\
%			\hline
			
%			firewire+deadline $\downarrow$ \\ (fix delay=3)
%			& deadline=14400
%			& deadline=14400
%			& deadline=14400 \\
%			\hline
%			
%			firewire+deadline $\downarrow$ \\ (fix deadline=200)
%			& delay=89
%      & delay=89
%      & delay=89 \\
%			\bottomrule
		\end{tabular}
	\end{adjustbox}
\end{table}


==> table-results-max-time.tex <==
\sisetup{round-mode=places,round-precision=2}
\begin{table}[t!]
	%\renewcommand{\arraystretch}{1.2}
	\setlength\fboxsep{1cm}
	\caption{
		The time for constructing and evaluating the decision tree for \emph{maximizing} properties.
%		%		\modes sometimes gives smaller value than optimal value (marked by $\sharp$)
%		%		as it uses SMC which does not report an exact value, but reports an approximate value (with $0.01$ error bound) with high ($99\%$) confidence.
%		The values marked by $\dagger$ were approximated using SMC.
%		We shorten the parameter deadline to \emph{dl}.
%		\oor \ means out-of-resources (both time and memory) and 
\rle \ means \emph{run length exceeded} given by \modes
%, an exception that occurs 
%		when the scheduler gets trapped in an end component.
	}
	\label{table:results:max:time}
	\begin{adjustbox}{width=1.2\textwidth,center}
	\begin{tabular}{p{0.3\textwidth}|lc|
			S[table-format=-1.2e-2,table-align-text-post=false] 
			S[table-format=-1.2e-2,table-align-text-post=false]
			S[table-format=-1.2e-2,table-align-text-post=false]
			HH
		}
		\toprule
		%			& && \multicolumn{5}{c}{\textbf{Time}}\\
		
		Model+property & \multicolumn{2}{c|}{\textbf{Scale}} & \multicolumn{3}{c}{\textbf{Time (s)}}\\
		
		(values~of~parameters) 
		& Variable
		& Time
		& {DT-construction}
		& {DT-evaluation}
		& {Smart LSS}
		& {Uniform}
		& {Random} \\\midrule
			
			
			\multirow{3}{*}{\parbox{0.3\textwidth}{zeroconf\_dl+deadline\_max \\	(N=1000, K=1)}}
			&	dl=200& \aminute  & 205.719   &  14.2  & 1.55  & 0.0029411764705882353 & 0.0007530000000000005 \\
			& dl=1600& \anhour  &  205.719  &  72.9  & 1.54  & 0.0012048192771084338 & 0.0006550000000000004 \\
			& dl=3200& Beyond  &  205.719  &  145.0  & 1.55  & 0 & 0.0006360000000000005 \\
			\midrule
			
			\multirow{3}{*}{\parbox{0.3\textwidth}{zeroconf\_dl+deadline\_max \\
					(N=1000, deadline=10)} }
			& K=2  & \aminute &  205.719 & 4.01 & 3.35 & 0.3429875518672199 & 0.3418300000000005\\
			& K=8  & \aminute &  205.719 & 4.62 & 4.10 & 1& 1 \\
			& K=32  & \aminute &  205.719 & 4.64 & 4.23 & 1& 1  \\
			\midrule
			
			\multirow{3}{*}{\parbox{0.3\textwidth}{zeroconf\_dl+deadline\_max  \\
					(deadline=10, K=1)} }
			& N=1000  & \aminute & 205.719 & 4.01 & 1.88 & 0.00909090909090909 & 0.006871999999999993\\
			& N=8000   & \aminute & 205.719 & 4.00 & 2.42 & 0.06748971193415639 & 0.06108600000000007\\
			& N=32000 & \aminute & 205.719 & 4.00 & 3.64 & 0.3471316549731738 & 0.3197710000000013\\
			\midrule
			
			\multirow{3}{*}{\parbox{0.3\textwidth}{philosophers+eat}}
			&N=5 & \aminute  &  1.307  &  .447  & 3.03  & 1 & 0.03734400000000001 \\
			&N=21& \anhour  &   1.307 &  1.35  & 12.7  & 1 & 0.000245 \\
			&N=34& Beyond  &   1.307 &   2.07 &  22.4 & 1 & 0 \\
			\midrule
			
			\multirow{3}{*}{\parbox{0.3\textwidth}{pnueli-zuck+live}}
			&N=5 &\aminute  &  0.415  & .785   & 4.24  & 1 & 0.035749 \\
			&N=21 &\anhour  &  0.415  & 7.99   & 37.4  & 1 & 0.002 \\
			&N=34 & Beyond  &  0.415  & 19.6   & 128.0  & 1 & 0.002 \\
			\midrule			
			
			\multirow{3}{*}{\parbox{0.3\textwidth}{csma+all\_before\_max \\ (N=2)}}
			& K=8 & \aminute  &  3.684  & 911.0   & 35.9  & 1 & 1 \\
			& K=11 & \anhour  &  3.684  &  321.0 {$^\dagger$}  & 171.0  & 1 & 1 \\
			& K=13 & Beyond  &  3.684  &  1200.0 {$^\dagger$} &  666.0 & 1 & \oor \\
			\midrule
			
			
			
			\multirow{3}{*}{\parbox{0.3\textwidth}{mer+p1 \\ (x=0.01)}}
			& n=1000& \aminute  &  1.027  & 0.375  & \rle  & \rle & 0.000184\\
			& n=21000 &\anhour  &  1.027  &  0.410  & \rle  & \rle  & 0\\
			& n=55000 & Beyond  &  1.027  & 0.375 & \rle  & \rle & 0.000399 \\
			\midrule
			
			\multirow{3}{*}{\parbox{0.3\textwidth}{mer+p1 \\ (n=10)}}
			& x=0.01  &  \aminute & 1.027  & 0.409  & \rle  & \rle  & 0.000402\\
			& x=0.08  & \aminute & 1.027   &  0.404  & \rle  & \rle & 0.000175\\
			& x=0.55  &  \aminute & 1.027  & 0.387 & \rle  & \rle  & 0.000494 \\
			& x=0.89 & \aminute  &  1.027  & 0.416  & \rle  & \rle & 0.0005809999999999999\\			
			\midrule
			
			
			\multirow{3}{*}{\parbox{0.3\textwidth}{consensus+disagree \\ (K=2)}}
			& N=5 & \aminute  &  0.392  &  1.71  &  36.1 & 0.029 & 0.03502900000000011 \\
			& N=7 &\anhour  &  0.392  &  5.28  &  108.0 & 0.043 & 0.03409800000000015 \\
			& N=13& Beyond  &  0.392  &  0.670  &  \rle & 0.03125 & \rle \\
			\midrule			
			
			\multirow{3}{*}{\parbox{0.3\textwidth}{consensus+disagree \\ (N=2)}}
			& K=2  & \aminute& 0.392  &  0.250 & 3.54 & 0.027887323943661974 & 0.027651000000000005\\
			& K=55  &  \aminute & 0.392 & 1.17 & \rle & \rle & \rle \\
			& K=144  &  \aminute& 0.392  &  3.58  &  \rle & \rle & \rle \\
			\midrule
			
			\multirow{3}{*}{\parbox{0.3\textwidth}{csma+all\_before\_max \\ (K=2)}}
			& N=3 &\aminute  &  3.684  &  4.60  & 16.8  & 0.032754342431761785 & 0.6838249999999996 \\
			& N=5 &\anhour  &  3.684  &  1220.0  &  48.9 & 0.0357308584686775 & 0.2363679999999993 \\
			& N=6& Beyond  &  3.684  & 1690.0{$^\dagger$}  & 49.7  & 0.03869565217391304 & 0.11185200000000006 \\
			%\midrule
			
			\bottomrule
		\end{tabular}
	\end{adjustbox}
\end{table}


==> table-results-min-time.tex <==
\sisetup{round-mode=places,round-precision=2}
\begin{table}[t!]
	%\renewcommand{\arraystretch}{1.2}
	%\setlength\fboxsep{1cm}
	\caption{
		The time for constructing and evaluating the decision tree for \emph{minimizing} properties. 
%		\modes sometimes gives smaller value than optimal value (marked by $\sharp$)
%		as it uses SMC which does not report an exact value, but reports an approximate value (with $0.01$ error bound) with high ($99\%$) confidence. For 1-2-3-Go, the values marked by $\dagger$ were approximated using SMC.
		We shorten the parameters delay to \emph{d}, deadline to \emph{dl}, and MAX\_STEPS to \emph{MS}.
		\oor\ means out-of-resources (both time and memory) and \rle\ means \emph{run length exceeded}, 
%		an exception that occurs 
%		when the scheduler gets trapped in an end component.
		an exception given by \modes.
	}
	\label{table:results:min:time}
	\begin{adjustbox}{width=1.2\textwidth,center}
			\begin{tabular}{p{0.3\textwidth}|lc|
					S[table-format=-1.2e-2,table-align-text-post=false] 
					H
					S[table-format=-1.2e-2,table-align-text-post=false]
					HH
				}
			\toprule
%			& && \multicolumn{5}{c}{\textbf{Time}}\\
			
			Model+property & \multicolumn{2}{c|}{\textbf{Scale}} & \multicolumn{3}{c}{\textbf{Time (s)}}\\
			
			(values~of~parameters) 
			& Variable
			& Time
			& {DT-construction}
			& {DT-evaluation}
			& {Smart LSS}
			& {Uniform}
			& {Random} \\\midrule
			
			\multirow{3}{*}{\parbox{0.3\textwidth}{zeroconf\_dl+deadline\_min\\
					(N=1000, K=1)}}
			& dl=200 &\aminute  &  184.823  & 8.42   & 3.52\notemodest  & 0.0029411764705882353 & 0.0006670000000000005 \\
			& dl=1600&\anhour  &  184.823  &  61.7  & 3.48  & 0.0012048192771084338 & 0.0006550000000000004 \\
			& dl=3200&Beyond  &  184.823  &  134.0  &  3.53 &  0 & 0.0007180000000000005 \\
			\midrule			
			
			\multirow{3}{*}{\parbox{0.3\textwidth}{zeroconf\_dl+deadline\_min\\
					(N=1000, deadline=10)} }
			& K=2 &\aminute &  184.823 & 2.04 & 2.89 & 0.3368200836820084\notemodest & 0.3422200000000006\\
			& K=8  & \aminute & 184.823 & 2.04 & 4.09 & 1& 1 \\[5pt]
			
%			&&& \multicolumn{5}{c}{\rednote{The model becomes trivial for K $>$ 3}} \\

			\midrule
			
			\multirow{3}{*}{\parbox{0.3\textwidth}{firewire+deadline\\ (deadline=200)}}
			& delay=5& \aminute &  0.657 & .743 & 11.1 & 0.99453125 & 0.9909990000000001\\
			&delay=21 &\aminute  & 0.657   &  .629  & 9.15  & 1 & 1 \\
			&delay=34 &\aminute  & 0.657   &  .644  & 8.1  & 1 & 1 \\
			&delay=89 &\aminute  &  0.657  &  .523  & 5.42  & 1 & 1 \\			
			\midrule
			
			\multirow{3}{*}{\parbox{0.3\textwidth}{firewire+deadline\\ (delay=3)}}
			& dl=200  &  \aminute & 0.657  &  .742  & 11.9\notemodest  & 0.9770491803278688 & 0.9709269999999999 \\
			& dl=500 & \aminute & 0.657 & 1.85 & 10.2 & 1 & 1\\
			& dl=1300 & \aminute& 0.657 & 9.42 & 9.94 & 1 & 1\\
			\midrule
			
			\multirow{3}{*}{\parbox{0.3\textwidth}{csma+some\_before\\ (N=2)}}
			& K=2 & \aminute  & 3.437  & .645  & 8.32\notemodest  & 0.49818799546998865\notemodest & 0.5003709999999995 \\
			& K=3 & \aminute  & 3.437  &  1.26  & 7.13  & 0.8726829268292683\notemodest & 0.8747569999999995\notemodest \\
			\midrule
			
			\multirow{3}{*}{\parbox{0.3\textwidth}{csma+some\_before\\ (fix K=2)}}
			& N=3 & \aminute  & 3.437  &  4.12  & 15.6\notemodest &  0.8944128787878788 & 0.9025649999999997 \\
			& N=5 & \anhour  &  3.437  &  957.00  & 54.8  & 0.7852764094143404 & 0.7778539999999998 \\
			& N=8 & \anhour  &  3.437  &  20392.09 {$^\dagger$}  & 167.00  & 0.7540229885057471 & 0.7602989999999993 \\
			& N=13 & Beyond  &  3.437 &  \oor  &  620.00 & 0.7527390438247012 & 0.7618870000000004 \\
			\midrule
					
			\multirow{3}{*}{\parbox{0.3\textwidth}{consensus+c2\\ (N=2)}}
			& K=2 & \aminute & 4.067  &  .348  & 5.36 & 0.4921509433962264 & 0.48594900000000113 \\
			& K=55  & \aminute &  4.067 &  .812 & \rle  & \rle & \rle \\
			& K=144  & \aminute & 4.067 &  1.65  & \rle  & \rle & \rle \\
			\midrule
			
			\multirow{3}{*}{\parbox{0.3\textwidth}{consensus+c2\\ (K=2)}}
			& N=6 &\aminute  & 4.067 &  2.06  & 89.0  & 0.48297470743676857 & 0.4831310000000007 \\
			& N=7 &\anhour  &  4.067 &  5.76 & 141.0  & 0.4858814647036618 & 0.48219200000000145 \\
			& N=13 & Beyond  &  4.067  &  467.0  &  \rle & 0.4858814647036618  &  \rle \\
			\midrule
			
			\multirow{3}{*}{\parbox{0.3\textwidth}{zeroconf\_dl+deadline\_min\\
					(deadline=10, K=1)} }
			& N=1000 &\aminute & 184.823 & 1.68 & 3.57& 0.007432432432432433\notemodest & 0.006983000000000012\\
			& N=8000  & \aminute & 184.823 & 1.65 & 1.68 & 0.07304236200256739 & 0.060227000000000086\\
			& N=32000 & \aminute& 184.823 & 1.63 & 3.12 & 0.31968900000000067  & 0.31968900000000067  \\
			\midrule
			
			
			\multirow{3}{*}{\parbox{0.3\textwidth}{pacman+crash}}
			& MS=5 &\aminute &  0.29 & 2.55 & 7.65\notemodest & 0.5494296577946768 & 0.5507580000000006\notemodest\\
			& MS=25  & \aminute & 0.29 & 4.49 & 18.9 & 0.9271557271557271 & 0.9226340000000002 \\
			& MS=200 & \anhour & 0.29 & 247.0 & 16.8 & 1 &  1 \\
			& MS=300 & Beyond & 0.29 & 396.0 & 17.1 & 1 & 1\\
			
			\bottomrule
		\end{tabular}
	\end{adjustbox}
\end{table}

